First observation of $B\!\to \bar{D}_1(\to\bar{D}\pi^+\pi^-)\ell^+\nu_\ell$ and measurement of the $B\!\to \bar{D}^{(*)}\pi\ell^+\nu_\ell$ and $B\!\to \bar{D}^{(*)}\pi^+\pi^-\ell^+\nu_\ell$ branching fractions with hadronic tagging at Belle

We report measurements of the ratios of branching fractions for $B \to \bar{D}^{(*)}\pi\ell^+\nu_\ell$ and $B \to \bar{D}^{(*)}\pi^+\pi^-\ell^+\nu_\ell$ relative to $B \to \bar{D}^*\ell^+\nu_\ell$ decays with $\ell = e, \mu$. These results are obtained from a data sample that contains $772 \times 10^6 B\bar{B}$ pairs collected near the $\Upsilon(4S)$ resonance with the Belle detector at the KEKB asymmetric energy $e^+e^-$ collider. Fully reconstructing both $B$ mesons in the event, we obtain \begin{align*} \frac{B(B^0 \to \bar{D}^0\pi^-\ell^+\nu_\ell)}{B(B^0 \to D^{*-}\ell^+\nu_\ell)} &= (7.24\pm0.36\pm0.12)\%\ ,\\ \frac{B(B^+ \to D^-\pi^+\ell^+\nu_\ell)}{B(B^+ \to \bar{D}^{*0}\ell^+\nu_\ell)} &= (6.78\pm0.24\pm0.15)\%\ ,\\ \frac{B(B^0 \to \bar{D}^{*0}\pi^-\ell^+\nu_\ell)}{B(B^0 \to D^{*-}\ell^+\nu_\ell)} &= (11.10\pm0.48\pm0.20)\%\ ,\\ \frac{B(B^+ \to D^{*-}\pi^+\ell^+\nu_\ell)}{B(B^+ \to \bar{D}^{*0}\ell^+\nu_\ell)} &= (9.50\pm0.33\pm0.27)\%\ ,\\ \frac{B(B^0 \to D^-\pi^+\pi^-\ell^+\nu_\ell)}{B(B^0 \to D^{*-}\ell^+\nu_\ell)} &= (2.91\pm0.37\pm0.25)\%\ ,\\ \frac{B(B^+ \to \bar{D}^0\pi^+\pi^-\ell^+\nu_\ell)}{B(B^+ \to \bar{D}^{*0}\ell^+\nu_\ell)} &= (3.10\pm0.26\pm0.21)\%\ ,\\ \frac{B(B^0 \to D^{*-}\pi^+\pi^-\ell^+\nu_\ell)}{B(B^0 \to D^{*-}\ell^+\nu_\ell)} &= (1.03\pm0.43\pm0.18)\%\ ,\\ \frac{B(B^+ \to \bar{D}^{*0}\pi^+\pi^-\ell^+\nu_\ell)}{B(B^+ \to \bar{D}^{*0}\ell^+\nu_\ell)} &= (1.25\pm0.27\pm0.15)\%\ , \end{align*} where the uncertainties are statistical and systematic, respectively. The invariant mass spectra of the $D\pi$, $D^*\pi$, and $D\pi\pi$ systems are studied. Branching fraction products are extracted, among them the first observations of $B(B^0 \to D_1^-\ell^+\nu_\ell) \times B(D_1^- \to D^-\pi^+\pi^-) = (0.102\pm0.013\pm0.009)\%$ and $B(B^+ \to \bar{D}_1^0\ell^+\nu_\ell) \times B(\bar{D}_1^0 \to \bar{D}^0\pi^+\pi^-) = (0.105\pm0.011\pm0.008)\%$.

==> pub629-plain.tex <==
%%% Paper:    B to D(*) pi (pi) l nu
%%% Journal:  Physical Review D
%%% Contacts: F. Meier
%%% Non-responding authors or those who said NO are commented out.
%%% ====================================================================
%%% Click the RELOAD button on your web browser to see the updated file.
%%% ====================================================================
%%% Use \input{author} to insert this material into your latex file.
%%%%% Force institutions to appear in alphabetical order when typeset.
\noaffiliation
  \author{F.~Meier} % Duke
  \author{A.~Vossen} % Duke
  \author{I.~Adachi} % KEK
  \author{K.~Adamczyk} % Ljubljana
% \author{J.~K.~Ahn} % Korea
  \author{H.~Aihara} % Tokyo
  \author{S.~Al~Said} % Tabuk
  \author{D.~M.~Asner} % BNL
  \author{H.~Atmacan} % Cincinnati
% \author{V.~Aulchenko} % BINP
  \author{T.~Aushev} % HSE
  \author{R.~Ayad} % Tabuk
% \author{T.~Aziz} % Tata
  \author{V.~Babu} % IJCLab
  \author{S.~Bahinipati} % IITB
% \author{A.~M.~Bakich} % Sydney
% \author{Y.~Ban} % Peking
  \author{Sw.~Banerjee} % Louisville
% \author{E.~Barberio} % Melbourne
% \author{M.~Barrett} % KEK
  \author{M.~Bauer} % Karlsruhe
  \author{P.~Behera} % IITM
  \author{K.~Belous} % Protvino
  \author{J.~Bennett} % Mississippi
  \author{F.~Bernlochner} % Bonn
  \author{M.~Bessner} % Hawaii
% \author{D.~Besson} % MEPhI
% \author{V.~Bhardwaj} % IISERM
  \author{B.~Bhuyan} % IITG
  \author{T.~Bilka} % Charles
% \author{S.~Bilokin} % LMU
  \author{D.~Biswas} % Louisville
  \author{A.~Bobrov} % BINP
  \author{D.~Bodrov} % HSE
% \author{A.~Bondar} % BINP
  \author{G.~Bonvicini} % WayneState
  \author{J.~Borah} % IITG
  \author{A.~Bozek} % Krakow
  \author{M.~Bra\v{c}ko} % Ljubljana
  \author{P.~Branchini} % RomaTre
% \author{N.~Braun} % Karlsruhe
  \author{T.~E.~Browder} % Hawaii
  \author{A.~Budano} % RomaTre
  \author{M.~Campajola} % Napoli
  \author{L.~Cao} % DESY
  \author{D.~\v{C}ervenkov} % Charles
  \author{M.-C.~Chang} % FuJen
  \author{P.~Chang} % Taiwan
% \author{V.~Chekelian} % MPI
  \author{A.~Chen} % NCU
% \author{C.~Chen} % ISU
% \author{Y.~Chen} % USTC
% \author{Y.-T.~Chen} % Taiwan
  \author{B.~G.~Cheon} % Hanyang
  \author{K.~Chilikin} % Lebedev
% \author{H.~E.~Cho} % Hanyang
  \author{K.~Cho} % KISTI
  \author{S.-J.~Cho} % Yonsei
  \author{S.-K.~Choi} % CAU
  \author{Y.~Choi} % Sungkyunkwan
  \author{S.~Choudhury} % ISU
  \author{D.~Cinabro} % WayneState
% \author{J.~Cochran} % ISU
% \author{S.~Cunliffe} % DESY
% \author{T.~Czank} % TMU
  \author{S.~Das} % MNIT
% \author{N.~Dash} % IITM
% \author{G.~de~Marino} % IJCLab
  \author{G.~De~Nardo} % Napoli
  \author{G.~De~Pietro} % Karlsruhe
  \author{R.~Dhamija} % IITH
  \author{F.~Di~Capua} % Napoli
  \author{J.~Dingfelder} % Bonn
  \author{Z.~Dole\v{z}al} % Charles
  \author{T.~V.~Dong} % DuyTan
% \author{D.~Dossett} % Melbourne
% \author{S.~Dubey} % Hawaii
% \author{P.~Ecker} % Karlsruhe
  \author{D.~Epifanov} % BINP
% \author{M.~Feindt} % Karlsruhe
  \author{T.~Ferber} % Karlsruhe
  \author{D.~Ferlewicz} % Melbourne
% \author{A.~Frey} % Goettingen
  \author{B.~G.~Fulsom} % PNNL
  \author{R.~Garg} % Panjab
  \author{V.~Gaur} % UPES
% \author{N.~Gabyshev} % BINP
% \author{A.~Garmash} % BINP
  \author{A.~Giri} % IITH
  \author{P.~Goldenzweig} % Karlsruhe
  \author{B.~Golob} % Ljubljana
% \author{G.~Gong} % USTC
  \author{E.~Graziani} % RomaTre
% \author{D.~Greenwald} % TUM
% \author{T.~Gu} % Pittsburgh
% \author{Y.~Guan} % Cincinnati
  \author{K.~Gudkova} % BINP
  \author{C.~Hadjivasiliou} % PNNL
  \author{S.~Halder} % Tata
% \author{X.~Han} % Beihang
% \author{K.~Hara} % KEK
  \author{T.~Hara} % KEK
% \author{O.~Hartbrich} % Hawaii
  \author{K.~Hayasaka} % Niigata
  \author{H.~Hayashii} % Nara
% \author{S.~Hazra} % Tata
  \author{M.~T.~Hedges} % Bonn
% \author{D.~Herrmann} % WayneState
% \author{M.~Hern\'{a}ndez~Villanueva} % DESY
% \author{T.~Higuchi} % IPMU
% \author{S.~Hirose} % Nagoya
  \author{W.-S.~Hou} % Taiwan
  \author{C.-L.~Hsu} % Sydney
% \author{K.~Huang} % Taiwan
% \author{T.~Iijima} % Nagoya
  \author{K.~Inami} % Nagoya
% \author{G.~Inguglia} % Vienna
  \author{N.~Ipsita} % IITH
  \author{A.~Ishikawa} % KEK
  \author{R.~Itoh} % KEK
  \author{M.~Iwasaki} % OsakaCity
% \author{Y.~Iwasaki} % KEK
% \author{S.~Iwata} % TMU
  \author{W.~W.~Jacobs} % Indiana
% \author{I.~Jaegle} % Florida
  \author{E.-J.~Jang} % Gyeongsang
% \author{H.~B.~Jeon} % Kyungpook
% \author{Q.~P.~Ji} % HNU
% \author{S.~Jia} % Fudan
  \author{Y.~Jin} % Trieste
% \author{C.~W.~Joo} % IPMU
% \author{K.~K.~Joo} % Chonnam
% \author{J.~Kahn} % Karlsruhe
% \author{H.~Kakuno} % TMU
% \author{D.~Kalita} % IITG
  \author{A.~B.~Kaliyar} % Vienna
  \author{K.~H.~Kang} % IPMU
% \author{S.~Kang} % ISU
% \author{P.~Kapusta} % Krakow
% \author{G.~Karyan} % DESY
% \author{Y.~Kato} % Nagoya
% \author{H.~Kawai} % Chiba
  \author{T.~Kawasaki} % Kitasato
% \author{H.~Kichimi} % KEK
  \author{C.~Kiesling} % MPI
% \author{B.~H.~Kim} % Seoul
  \author{C.~H.~Kim} % Hanyang
  \author{D.~Y.~Kim} % Soongsil
% \author{H.~J.~Kim} % Kyungpook
  \author{K.-H.~Kim} % KISTI
% \author{K.~T.~Kim} % Korea
% \author{S.~H.~Kim} % Seoul
% \author{S.~K.~Kim} % Seoul
% \author{Y.~J.~Kim} % Korea
  \author{Y.-K.~Kim} % Yonsei
% \author{T.~D.~Kimmel} % VPI
% \author{H.~Kindo} % VPI
  \author{K.~Kinoshita} % Cincinnati
% \author{C.~Kleinwort} % DESY
  \author{P.~Kody\v{s}} % Charles
% \author{I.~Komarov} % DESY
% \author{T.~Konno} % Kitasato
  \author{A.~Korobov} % BINP
  \author{S.~Korpar} % Ljubljana
  \author{E.~Kovalenko} % BINP
  \author{P.~Kri\v{z}an} % Ljubljana
  \author{R.~Kroeger} % Mississippi
% \author{J.-F.~Krohn} % Melbourne
  \author{P.~Krokovny} % BINP
  \author{T.~Kuhr} % LMU
  \author{M.~Kumar} % MNIT
  \author{R.~Kumar} % Punjab
  \author{K.~Kumara} % Mississippi
% \author{T.~Kumita} % TMU
% \author{E.~Kurihara} % Chiba
% \author{A.~Kuzmin} % BINP
% \author{P.~Kvasni\v{c}ka} % Charles
  \author{Y.-J.~Kwon} % Yonsei
% \author{Y.-T.~Lai} % IPMU
% \author{K.~Lalwani} % MNIT
  \author{T.~Lam} % VPI
  \author{J.~S.~Lange} % Giessen
% \author{M.~Laurenza} % RomaTre
% \author{I.~S.~Lee} % Hanyang
% \author{J.~K.~Lee} % Seoul
  \author{S.~C.~Lee} % Kyungpook
% \author{D.~Levit} % KEK
  \author{P.~Lewis} % Bonn
  \author{C.~H.~Li} % LNNU
% \author{J.~Li} % Kyungpook
  \author{L.~K.~Li} % Cincinnati
% \author{S.~X.~Li} % Fudan
  \author{Y.~Li} % Fudan
  \author{Y.~B.~Li} % Fudan
  \author{L.~Li~Gioi} % MPI
  \author{J.~Libby} % IITM
  \author{K.~Lieret} % LMU
  \author{Y.-R.~Lin} % Taiwan
% \author{Z.~Liptak} % Hiroshima
  \author{D.~Liventsev} % WayneState
% \author{A.~Loos} % SouthCarolina
  \author{T.~Luo} % Fudan
% \author{J.~MacNaughton} % NPC
% \author{A.~Martini} % DESY
  \author{M.~Masuda} % NPC
  \author{T.~Matsuda} % NPC
  \author{D.~Matvienko} % BINP
  \author{S.~K.~Maurya} % IITG
% \author{J.~T.~McNeil} % Florida
  \author{M.~Merola} % Napoli
  \author{F.~Metzner} % Bonn
  \author{K.~Miyabayashi} % Nara
% \author{H.~Miyake} % KEK
% \author{H.~Miyata} % Niigata
  \author{R.~Mizuk} % Lebedev
% \author{G.~B.~Mohanty} % Tata
% \author{S.~Mohanty} % Tata
% \author{H.~K.~Moon} % Korea
% \author{T.~J.~Moon} % Seoul
% \author{H.-G.~Moser} % MPI
% \author{M.~Mrvar} % Vienna
% \author{T.~M\"uller} % Karlsruhe
  \author{R.~Mussa} % Torino
  \author{I.~Nakamura} % KEK
% \author{K.~R.~Nakamura} % KEK
% \author{E.~Nakano} % OsakaCity
% \author{T.~Nakano} % NPC
  \author{M.~Nakao} % KEK
% \author{H.~Nakayama} % KEK
% \author{H.~Nakazawa} % Taiwan
% \author{D.~Narwal} % IITG
  \author{Z.~Natkaniec} % Krakow
  \author{A.~Natochii} % Hawaii
  \author{L.~Nayak} % IITH
  \author{M.~Nayak} % TelAviv
% \author{C.~Niebuhr} % DESY
% \author{M.~Niiyama} % NPC
  \author{N.~K.~Nisar} % BNL
  \author{S.~Nishida} % KEK
% \author{K.~Nishimura} % Hawaii
% \author{K.~Ogawa} % Niigata
  \author{S.~Ogawa} % Toho
% \author{S.~Okuno} % Kanagawa
% \author{S.~L.~Olsen} % CAU
  \author{H.~Ono} % NihonDental
% \author{Y.~Onuki} % Tokyo
  \author{P.~Oskin} % Lebedev
% \author{H.~Ozaki} % KEK
  \author{P.~Pakhlov} % Lebedev
  \author{G.~Pakhlova} % HSE
% \author{T.~Pang} % Pittsburgh
  \author{S.~Pardi} % Napoli
  \author{H.~Park} % Kyungpook
  \author{J.~Park} % Yonsei
% \author{S.-H.~Park} % KEK
  \author{A.~Passeri} % RomaTre
  \author{S.~Patra} % IISERM
  \author{S.~Paul} % TUM
% \author{T.~K.~Pedlar} % Luther
  \author{R.~Pestotnik} % Ljubljana
% \author{F.~Pham} % Melbourne
  \author{L.~E.~Piilonen} % VPI
  \author{T.~Podobnik} % Ljubljana
% \author{V.~Popov} % HSE
% \author{S.~Prell} % ISU
  \author{E.~Prencipe} % Giessen
  \author{M.~T.~Prim} % Bonn
% \author{M.~V.~Purohit} % OIST
% \author{A.~Rabusov} % TUM
% \author{P.~K.~Resmi} % IITM
% \author{M.~Ritter} % LMU
% \author{M.~R\"{o}hrken} % DESY
  \author{A.~Rostomyan} % DESY
  \author{N.~Rout} % IITM
% \author{M.~Rozanska} % Krakow
  \author{G.~Russo} % Napoli
% \author{D.~Sahoo} % ISU
% \author{Y.~Sakai} % KEK
% \author{M.~Salehi} % Malaya
  \author{S.~Sandilya} % IITH
% \author{A.~Sangal} % Cincinnati
  \author{L.~Santelj} % Ljubljana
% \author{T.~Sanuki} % Tohoku
% \author{Y.~Sato} % KEK
  \author{V.~Savinov} % Pittsburgh
% \author{P.~Schmolz} % LMU
% \author{O.~Schneider} % Lausanne
  \author{G.~Schnell} % Bilbao
% \author{J.~Schueler} % Hawaii
  \author{C.~Schwanda} % Vienna
  \author{A.~J.~Schwartz} % Cincinnati
% \author{B.~Schwenker} % Goettingen
% \author{R.~Seidl} % RIKEN
  \author{Y.~Seino} % Niigata
  \author{K.~Senyo} % Yamagata
% \author{O.~Seon} % Nagoya
% \author{I.~S.~Seong} % Hawaii
  \author{M.~E.~Sevior} % Melbourne
% \author{W.~Shan} % HUNNU
  \author{M.~Shapkin} % Protvino
  \author{C.~Sharma} % MNIT
% \author{V.~Shebalin} % Hawaii
  \author{C.~P.~Shen} % Fudan
% \author{H.~Shibuya} % Toho
  \author{J.-G.~Shiu} % Taiwan
% \author{B.~Shwartz} % BINP
% \author{A.~Sibidanov} % Hawaii
  \author{F.~Simon} % MPI
  \author{J.~B.~Singh} % Panjab
% \author{R.~Sinha} % IMSC
% \author{K.~Smith} % Melbourne
  \author{A.~Soffer} % TelAviv
% \author{A.~Sokolov} % Protvino
% \author{Y.~Soloviev} % DESY
  \author{E.~Solovieva} % Lebedev
% \author{S.~Stani\v{c}} % NovaGorica
  \author{M.~Stari\v{c}} % Ljubljana
  \author{Z.~S.~Stottler} % VPI
  \author{J.~F.~Strube} % PNNL
% \author{J.~Stypula} % Krakow
  \author{M.~Sumihama} % NPC
% \author{K.~Sumisawa} % KEK
  \author{T.~Sumiyoshi} % TMU
% \author{W.~Sutcliffe} % Bonn
% \author{S.~Y.~Suzuki} % KEK
  \author{M.~Takizawa} % NPC
  \author{U.~Tamponi} % Torino
% \author{S.~Tanaka} % KEK
% \author{S.~S.~Tang} % Fudan
  \author{K.~Tanida} % NPC
% \author{N.~Taniguchi} % KEK
% \author{Y.~Tao} % Florida
% \author{G.~N.~Taylor} % Melbourne
  \author{F.~Tenchini} % Pisa
% \author{Y.~Teramoto} % OsakaCity
% \author{A.~Thampi} % Juelich
% \author{R.~Tiwary} % Tata
  \author{K.~Trabelsi} % IJCLab
% \author{T.~Tsuboyama} % KEK
  \author{M.~Uchida} % NPC
% \author{I.~Ueda} % KEK
% \author{S.~Uehara} % KEK
  \author{T.~Uglov} % Lebedev
  \author{Y.~Unno} % Hanyang
  \author{K.~Uno} % Niigata
  \author{S.~Uno} % KEK
  \author{P.~Urquijo} % Melbourne
% \author{Y.~Ushiroda} % KEK
% \author{Y.~Usov} % BINP
  \author{S.~E.~Vahsen} % Hawaii
  \author{R.~Van~Tonder} % Bonn
  \author{G.~Varner} % Hawaii
  \author{K.~E.~Varvell} % Sydney
  \author{A.~Vinokurova} % BINP
% \author{V.~Vorobyev} % BINP
% \author{E.~Waheed} % KEK
% \author{B.~Wang} % MPI
% \author{C.~H.~Wang} % NUU
% \author{D.~Wang} % Florida
% \author{E.~Wang} % Pittsburgh
  \author{M.-Z.~Wang} % Taiwan
% \author{X.~L.~Wang} % Fudan
  \author{M.~Watanabe} % Niigata
% \author{Y.~Watanabe} % Kanagawa
  \author{S.~Watanuki} % Yonsei
% \author{S.~Wehle} % DESY
% \author{O.~Werbycka} % Trieste
% \author{E.~Widmann} % Vienna
  \author{J.~Wiechczynski} % Krakow
  \author{E.~Won} % Korea
  \author{X.~Xu} % Soochow
  \author{B.~D.~Yabsley} % Sydney
% \author{S.~Yamada} % KEK
% \author{H.~Yamamoto} % Tohoku
  \author{W.~Yan} % USTC
  \author{S.~B.~Yang} % Korea
% \author{H.~Ye} % DESY
% \author{J.~Yelton} % Florida
  \author{J.~H.~Yin} % Korea
% \author{Y.~Yook} % IHEP
  \author{C.~Z.~Yuan} % IHEP
  \author{L.~Yuan} % Beihang
  \author{Y.~Yusa} % Niigata
% \author{Y.~Zhai} % ISU
% \author{J.~Zhang} % IHEP
  \author{Z.~P.~Zhang} % USTC
% \author{V.~Zhilich} % BINP
  \author{V.~Zhukova} % Lebedev
% \author{V.~Zhulanov} % BINP
\collaboration{The Belle Collaboration}

